Characteristic classes and stability conditions for projective Kleinian orbisurfaces

We construct Bridgeland stability conditions on the derived category of smooth quasi-projective Deligne-Mumford surfaces whose coarse moduli spaces have ADE singularities. This unifies the construction for smooth surfaces and Bridgeland's work on Kleinian singularities. The construction hinges on an orbifold version of the Bogomolov-Gieseker inequality for slope semistable sheaves on the stack, and makes use of the To\"en-Hirzebruch-Riemann-Roch theorem.

==> TRR.tex <==
\section{Applications of To\"en--Riemann--Roch}

The goal of this appendix is to obtain formulae for the correction term appearing in Theorem \ref{thm:tgrr}. This extends the computation  done in \cite{Lie11} for singularities of type $A$, and completes the one started in \cite{CT19}, where the authors only compute a special case.

 Keeping the notation as above, we have
\[ \delta(F)= \sum\limits_{(g)\neq (I)} \frac{1}{\abs{C_G(g)}}\cdot\frac{\sum_ia_i\chi_i(g)}{2-\chi_V(g)}=
\sum_i a_i T_i,\]
with 
\begin{equation}\label{eq_formula_for_Ti}
  T_i\coloneqq  \sum\limits_{(g)\neq (I)} \frac{\chi_i(g)}{\abs{C_G(g)}(2-\chi_V(g))}  
\end{equation}
only depending on the character table of $G$. Next, we give explicit expressions for the coefficients $T_i$ for all kleinian singularities. 

\subsection{Singularities of type $A$} In this case, the coefficients $T_j$ are computed by Lieblich in \cite[Sec. 3.3.2]{Lie11}, who gives an explicit formula for $\delta(F)$. We recall his result here. We'll make use of the following Lemma:
\begin{lemma}[{\cite[Lemma 3.3.2.1]{Lie11}}]\label{lem_Lieblich}
Let $\zeta$ be a primitive $P$-th root of unity and $j\leq P$ a non-negative integer. Then
\[ \sum\limits_{k=1}^{P-1}\frac{\zeta^{kj}}{2-\zeta^k -\zeta^{-k}}=\frac{j(j-P)}{2} + \frac{P^2-1}{12}. \]
\end{lemma}

The \(K\)-theory of \(B\mu_N\) is free Abelian of rank $N$ with $\{ \chi^j \,|\,j=0,...,N-1 \}$ 
%\({\bf 1}\) and \(\chi\) 
as a basis. For any perfect complex of sheaves \(\sF\) on \(\sS\), we
have
\[
    [{\bf L}\iota_u^\ast\sF] = \sum_{j=0}^{N-1} a_j\chi^j.
\]
Define a function $f\colon \Z/N\Z \to \Q$ by the formula
\[ f(\overline{x})=\frac{x(x-N)}{2} + \frac{N^2-1}{12}. \]

Let $\zeta\in G$ be a primitive $N$-th root of unity. It acts on $\chi^j$ with multiplication by $\zeta^j$. Then, equation \eqref{eq_formula_for_Ti} reads
\[ T_j = \frac 1N \sum\limits_{k=1}^{N-1}\frac{\zeta^{kj}}{2-\zeta^k -\zeta^{-k}} =\frac 1N f(j) \]
as a consequence of Lemma \ref{lem_Lieblich}.

%For the complex $\sF$, we have
%\[ \delta(\sF)=\frac 1N\sum\limits_{j=0}^{N-1}f(j)a_j. \]


\begin{comment}
\begin{example}\AAA{Possibly just remove completely}
The group acting in this case is $G=\mu_N$, let $\chi$ be a generator for the character group. Since $G$ is abelian of order $N$, Lemma \ref{lem_delta_of_skyscrapers} implies $\ch{2}(\sO_p)=\ch{2}(\sO_p\chi^j)=1/N$ and $\delta(\sO_p)=1-1/N$ and $\delta(\sO_p\chi^j)=-1/N$. 

Moreover,  $\ch{}(\sO)=(1,0,0)$ and $D\coloneqq\delta(\sO)=\frac{N^2-1}{12N}$.

If we consider 
\[ \mathfrak m \to \sO \to \sO_p \]
we obtain $\ch{}(\mathfrak m)=(1,0,-1/N)$ and $\delta(\mathfrak m)=D- 1+ 1/N$. 

If for example $N=2$, we can further write  
\[ \pi^*\pi_*\mathfrak m=I_p \to \mathfrak m\to \sO_{p}\chi \]
and observe $\ch{}(I_p)=(1,0,-N/N)$ and $\delta(I_p)= \delta(\mathfrak m) - \delta(\sO_p\chi)=D - 1+1/N + (N-1)( 1/N) = D $.
\end{example}



\AAA{remove/rewrite?} We now give a few more examples in the case of surfaces with a singularity of type D or E. Recall that the fundamental cycle of the singularity, $C$, is the smallest effective cycle such that $C.C_i\leq 0$ for all irreducible exceptional curves $C_i$. If the irreducible representation $\rho_i$ corresponds to the exceptional curve $C_i$, then $C_i$ appears in $C$ with multiplicity $r_i\coloneqq \dim \rho_i$.
\end{comment}

\subsection{Singularities of type $D$: Binary dihedral groups} In this case, the group acting is the binary dihedral group $G=Dic_n$, it has order $4n$. We can present it as 
\[ Dic_n=\pair{a,x \,\lvert\, a^{2n}=I, x^2=a^n, x^{-1}ax=a^{-1}}. \]
The center of $G$ is cyclic of order 2, generated by $x^2=a^n$. The quotient of $G$ by its center is the dihedral group $D_n$ with $2n$ elements. 

The group $G$ has $n+3$ conjugacy classes, grouped by cardinality as: 
\begin{align*}
  \set{I},  \set{-I=x^2=a^n}\\
  \set{a,a^{-1}}, \set{a^2,a^{-2}}, ... \set{a^{n-1},a^{n+1}},\\
  \set{xa,xa^3,...,xa^{2n-2}}, \set{x,xa^2,...,xa^{2n-1}}.
\end{align*}
The corresponding centralizers have cardinality $4n$, $2n$ and $4$.

There are 4 one-dimensional representations. In addition to these, there are two-dimensional representations, called \textit{dihedral}, induced by $G\to D_n$ there are $\frac{n-1}{2}$ of these if $n$ is odd, and $\frac{n-2}{2}$ if $n$ is even. The $l$-th dihedral representation is given by the assignment
\[ a\mapsto\begin{pmatrix} e^{\frac{2l\pi i}{n}} & 0\\ 0 & e^{-\frac{2l\pi i}{n}} \end{pmatrix}; \qquad x=\begin{pmatrix} 0 & 1\\ 1 & 0 \end{pmatrix}. \]

 The remaining representations are called of \textit{quaternionic type} since they are induced by an inclusion $G\subset \SL(2,\C)$. They are also two-dimensional, there are $\frac{n-1}{2}$ if $n$ is odd, or $\frac n2$ if $n$ is even. The $l$-th quaternionic representation is given by  
 \[ a\mapsto\begin{pmatrix} e^{\frac{l\pi i}{n}} & 0\\ 0 & e^{-\frac{l\pi i}{n}} \end{pmatrix}; \qquad x=\begin{pmatrix} 0 & -1\\ 1 & 0 \end{pmatrix}. \]
We assume that $G$ acts on $\C^2$ via the first ($l=1$) quaternionic representation, and denote by $V$ this representation. 
%The fundamental cycle for a singularity of type $D$ has coefficient 2 for all irreducible curves except the three terminal ones. 

Let $T_\rho$ the coefficent corresponding to a representation $\rho$ as in \eqref{eq_formula_for_Ti}. For $G=Dic_n$, we have
\[ T_\rho = -\frac{\dim \rho}{16n} + \frac 18(\chi_\rho(x)+\chi_\rho(xa)) + \frac{1}{2n}\sum_{k=1}^{n-1}\frac{\chi_\rho(a^k)}{2-\chi_V(a^k)}. \]


First, we compute coefficients for the 4 one-dimensional representations. Let $\rho_x$ be the representation where $x$ acts by -1 and everything else acts trivially, similarly for $\rho_a$ and $\rho_{x,a}$. Let $\zeta\coloneqq e^{-\frac{\pi i}{n}}$. By applying Lemma \ref{lem_Lieblich} we obtain
\begin{align}
T_{\mathbbm 1}&= -\frac{1}{16n} + \frac 14 + \frac{n^2-1}{12n}\\
        T_{\rho_x}&= -\frac{1}{16n} - \frac 14 + \frac{n^2-1}{12n}.    \end{align}
The remaining coefficient is 
\begin{equation}\label{eq_express T_a}
T_{\rho_a}= T_{\rho_{x,a}}= -\frac{1}{16n} + \frac{1}{2n}\sum_{k=1}^{n-1}\frac{(-1)^k}{2-\chi_V(a^k)}=-\frac{1}{16n} + \frac{1}{2n}\sum_{k=1}^{n-1}\frac{\zeta^{nk}}{2-\zeta^k-\zeta^{-k}}.
\end{equation}
Now we compute the the sum in \eqref{eq_express T_a}: substituting $h=2n-k$ we have
\begin{equation}\label{eq_substitute_hk}
    \begin{split}
    \sum_{k=1}^{n-1}\frac{\zeta^{-kl}}{\left(2-\zeta^k-\zeta^{-k}\right)}= \sum_{h=n+1}^{2n-1}\frac{\zeta^{(h-2n)l}}{\left(2-\zeta^{2n-h}-\zeta^{h-2n}\right)}= \sum_{h=n+1}^{2n-1}\frac{\zeta^{hl}}{\left(2-\zeta^{-h}-\zeta^{h}\right)}.
    \end{split}
\end{equation}
Using the \eqref{eq_substitute_hk} with $l=n$, write
\begin{equation*}
     \sum_{k=1}^{2n-1}\frac{\zeta^{nk}}{\left(2-\zeta^k-\zeta^{-k}\right)} = \sum_{k=1}^{n-1}\frac{\zeta^{nk}}{\left(2-\zeta^k-\zeta^{-k}\right)} + \frac{(-1)^n}{4} + \sum_{k=1}^{n-1}\frac{\zeta^{-nk}}{\left(2-\zeta^k-\zeta^{-k}\right)}.
     \end{equation*}
whence, applying Lemma \ref{lem_Lieblich} with $P=2n$ and $j=n$,
\begin{equation*}
\begin{split}
\sum_{k=1}^{n-1}\frac{\zeta^{nk}}{\left(2-\zeta^k-\zeta^{-k}\right)}= \frac 12 \left[     \sum_{k=1}^{2n-1}\frac{\zeta^{nk}}{\left(2-\zeta^k-\zeta^{-k}\right)} - \frac{(-1)^n}{4} \right] = \\
\frac 12 \left[    -\frac{n^2}{2} + \frac{4n^2-1}{12} - \frac{(-1)^n}{4} \right].
\end{split}
     \end{equation*}
    
If $\sigma$ is the $l$-th quaternionic representation, we have 
\begin{equation}
 T_\sigma = -\frac{1}{8n} +  \frac{1}{2n}\sum_{k=1}^{n-1}\frac{\left(\zeta^{kl}+\zeta^{-kl}\right)}{\left(2-\zeta^k-\zeta^{-k}\right)}. 
\end{equation}
Using once again the substitution \eqref{eq_substitute_hk}, we obtain:
\begin{equation*}
    \begin{split}
     \sum_{k=1}^{n-1}\frac{\left(\zeta^{kl}+\zeta^{-kl}\right)}{\left(2-\zeta^k-\zeta^{-k}\right)} = \sum_{k=1}^{n-1}\frac{\zeta^{kl}}{\left(2-\zeta^k-\zeta^{-k}\right)} + \sum_{k=1}^{n-1}\frac{\zeta^{-kl}}{\left(2-\zeta^k-\zeta^{-k}\right)}=\\
     \sum_{k=1}^{n-1}\frac{\zeta^{kl}}{\left(2-\zeta^k-\zeta^{-k}\right)} + \sum_{h=n+1}^{2n-1}\frac{\zeta^{hl}}{\left(2-\zeta^{-h}-\zeta^{h}\right)}= \sum_{k=1}^{2n-1}\frac{\zeta^{kl}}{\left(2-\zeta^{-k}-\zeta^{k}\right)} - \frac{(-1)^l}{4}.
    \end{split}
\end{equation*}
Applying Lemma \ref{lem_Lieblich} with $P=2n$ and $j=l$ then yields
\begin{equation*}
    \begin{split}
     \sum_{k=1}^{n-1}\frac{\left(\zeta^{kl}+\zeta^{-kl}\right)}{\left(2-\zeta^k-\zeta^{-k}\right)} = \frac{l(l-2n)}{2} + \frac{(2n)^2-1}{12}- \frac{(-1)^l}{4},
    \end{split}
\end{equation*}
and finally
\begin{equation}
T_\sigma = -\frac{1}{8n} +  \frac{1}{2n}\left( -\frac {(-1)^l}4 + \frac{l(l-2n)}{2} + \frac{(2n)^2-1}{12} \right). 
\end{equation}

If $\tau$ is a dihedral representation, then
\begin{equation}
T_\tau = -\frac{1}{8n} +  \frac{1}{2n}\sum_{k=1}^{n-1}\frac{\left(\zeta^{2kl}+\zeta^{-2kl}\right)}{\left(2-\zeta^{k}-\zeta^{-k}\right)} 
\end{equation}
and we may repeat the argument above applying Lemma \ref{lem_Lieblich} with $P=2n$ and $j=2l$:
\begin{equation}
\frac{1}{2n}\sum_{k=1}^{n-1}\frac{\left(\zeta^{2kl}+\zeta^{-2kl}\right)}{\left(2-\zeta^{k}-\zeta^{-k}\right)}=
\left( -\frac {1}4 + 2l(l-n) + \frac{(2n)^2-1}{12} \right).
\end{equation}

\subsubsection{Example: the $D_4$ singularity} The binary dihedral group $G=Dic_n$ with $n=2$ has order $4n=8$. We present it as the group of matrices generated by 
\[ a=\begin{pmatrix} i & 0\\ 0 & -i \end{pmatrix}; \qquad x=\begin{pmatrix} 0 & -1\\ 1 & 0 \end{pmatrix}. \]

As above, let $\mathbf 1, \rho_a, \rho_x$ and $\rho_{xa}$ denote the one-dimensional representations. The two dimensional irreducible representation is denoted $V$.

For a sheaf $F$ we can write $[Li^*F]=\sum_{\rho}a_\rho \rho.$

Then the correction term is 
\[ \delta(F)= \sum_{\rho} a_\rho T_\rho \]
with $T_{\mathbbm 1}=\frac{13}{32}$, $T_{\rho_a}=T_{\rho_x}=T_{\rho_{xa}}=-\frac{3}{32}$ and $T_V=-\frac{2}{32}$.

As an example, we explicitly check Lemma \ref{lem_delta_of_skyscrapers} in a few cases. Let $F=\sO_p$. Then we have $[Li^*\sO_p]= 2\mathbf{1}-V$. Plugging this in, we get 
\[ \delta(\sO_p)=2\cdot\frac{13}{32} - \frac{-2}{32}= \frac 78. \]
%(the first denominator of each summand is the order of the centralizer, the second is the term $2-\xi_g-\xi_g^{-1}$, which is computed in \cite{CT19}). Note moreover that $\ch 2(\sO_p)=\frac18$, and these two added together give exactly $\chi(\sO_p)=1$. 
%The denominator 8 is a bit unexpected to me, but I guess it makes sense if we believe that the (untwisted part of the) Chern character of $\sO_pV$ is $\frac12$, 4 times that of $\sO_p\chi$ where $\chi$ is any character. So that when you add them together you get that the second chern character of a cluster is exactly 1.
%\end{example}

%\begin{example}
Now let $F=\sO_p\otimes V$. Observe that $V\otimes V = \oplus_{j=0}^3 \chi^j$, whence $[Li^*\sO_p]= 2V-(\sum \chi^j)$, i.e. $a_0=...=a_3=-1$ and $a_4=2$. The same computation as above yields $\delta(\sO_p\otimes V)=-\frac 14$.


\begin{comment}
(Follow notation and computations from \cite{CT19}) In this case, the group acting is the binary dihedral group $G=Dic_n$ with $n=2$, it has order $4n=8$. We can present it as the group of matrices generated by 
\[ a=\begin{pmatrix} i & 0\\ 0 & -i \end{pmatrix}; \qquad x=\begin{pmatrix} 0 & -1\\ 1 & 0 \end{pmatrix}. \]

One obtains the 4 characters by quotienting out by $a^2$. We label them $\mathbf 1, \chi_1,\chi_2,\chi_3=\chi_1\otimes\chi_2$. Let's use the convention that $a$ acts non-trivially on $\chi_1$ and $x$ does likewise on $\chi_2$. In addition to these there is the natural irreducible representation $V$.

$G$ admits 5 conjugacy classes: 
\[  \set{I}, \set{-I}, \set{a,a^{-1}}, \set{xa,xa^3}, \set{x,xa^2}\]
The centralizer of the first 2 has order 8, and 4 for the last three. 

Let $F$ be a sheaf on $\sS$, then we can write $[Li^*F]=a_0\mathbf{1}+ \sum a_i\chi^i+a_4V.$

Now, I claim that the Riemann-Roch contribution to $\chi(F)$ coming from the piece $Li^*F_{|BC_G(g)}$ is computed looking at the eigenvalues of the action of $g$ on $[Li^*F]$ as follows.

\begin{itemize}
    \item $g\in (-I)$. This element acts trivially (with eigenvalue 1) on all characters, and with eigenvalue -1 (repeated) on $V$. Hence, \[ \widetilde{\ch{}}(F_{|BC_G(-I)})=(a_0+a_1+...+a_3 -a_4-a_4)=(a_0+...+a_3-2a_4). \]
    \item $g\in (a)$ (wlog $g=a$) acts by negating $\chi_1$ and $\chi_3$, trivially on the others, and with eigenvalues $i$ and $-i$ on $V$. Hence its contribution is
    \[ \widetilde{\ch{}}(F_{|BC_G(a)})=(a_0-a_1+a_2 -a_3 +a_4(i-i))=(a_0-a_1+a_2-a_3). \]
    \item $g=xa$ acts non-trivially on $\chi_1$ and $\chi_2$, and with eigenvalues $\pm i$ on $V$. Hence
    \[ \widetilde{\ch{}}(F_{|BC_G(xa)})=(a_0-a_1-a_2 +a_3). \]
    \item $g=x$ acts non-trivially on $\chi_2$ and $\chi_3$, and with $\pm i$ on $V$. Again, 
     \[ \widetilde{\ch{}}(F_{|BC_G(x)})=(a_0+a_1-a_2 -a_3). \]
\end{itemize}
This exhausts all contributions. Then the correction term is 
\[ \delta(F)=  \sum\limits_{(g)\neq (I)} \frac{1}{\abs{C_G(g)}}\cdot\frac{\widetilde{\ch{}}(F_{|BC_G(g)})}{2-\chi_V(g)}= \sum_{i=0}^4 a_i T_i \]
with $T_0=\frac{13}{32}$, $T_1=T_2=T_3=-\frac{3}{32}$ and $T_4=-\frac{2}{32}$, computed as in Remark \ref{rmk_formulaeT_i}.

\begin{example} We explicitly check Lemma \ref{lem_delta_of_skyscrapers} in a few cases. Let $F=\sO_p$. Then we have $[Li^*\sO_p]= 2\mathbf{1}-V,$ i.e. $a_0=2$, $a_4=-1$ and $a_i=0$ else. Plugging this in, we get 
\[ \delta(\sO_p)=2\cdot\frac{13}{32} - \frac{-2}{32}= \frac 78. \]
%(the first denominator of each summand is the order of the centralizer, the second is the term $2-\xi_g-\xi_g^{-1}$, which is computed in \cite{CT19}). Note moreover that $\ch 2(\sO_p)=\frac18$, and these two added together give exactly $\chi(\sO_p)=1$. 
%The denominator 8 is a bit unexpected to me, but I guess it makes sense if we believe that the (untwisted part of the) Chern character of $\sO_pV$ is $\frac12$, 4 times that of $\sO_p\chi$ where $\chi$ is any character. So that when you add them together you get that the second chern character of a cluster is exactly 1.
%\end{example}

%\begin{example}
Now let $F=\sO_p\otimes V$. Observe that $V\otimes V = \oplus_{j=0}^3 \chi^j$, whence $[Li^*\sO_p]= 2V-(\sum \chi^j)$, i.e. $a_0=...=a_3=-1$ and $a_4=2$. The same computation as above yields $\delta(\sO_p\otimes V)=-\frac 14$.
\end{example}
\end{comment}


\subsection{Singularities of type E}
The groups giving rise to singularities of type $E$ are the binary tetrahedral ($E_6$), binary octahedral ($E_7$) and binary icosahedral group ($E_8$).

The binary tetrahedral group $2T$ has 24 elements, and it can be identified with the following quaternion numbers:
\[ \frac{1}{2}(\pm 1\pm i \pm j \pm k), \qquad \pm 1,\qquad \pm i, \qquad \pm j, \qquad \pm k. \]
It has 7 conjugacy classes and 6 non-trivial irreducible representations. Let $\omega\coloneqq e^{\frac{2\pi i}{3}}$ denote a third root of unity, and consider the elements $a=\frac12(1+i+j+k)$, $b=\frac12(1+i+j-k)$, $c=\frac12(-1+i+j+k)$ and $d=\frac12(-1+i+j-k)$. Then the character table of $2T$ is:
\begin{center}
\begin{tabular}{c|ccccccc}
 & $1$ & $-1$ & $i$ & $a$ & $b$ & $c$ & $d$ \\
 \hline
$\abs{C_G(g)}$ & 24 & 24 & 4 & 6 & 6 & 6 & 6\\
\hline
$\rho_0$& $1$ & $1$ & $1$ & $1$ & $1$ & $1$ & $1$ \\
$\rho_1$ & $1$ & $1$ & $1$ & $\omega$ & $\omega^2$ & $\omega^2$ & $\omega$ \\
$\rho_2$ & $1$ & $1$ & $1$ & $\omega^2$ & $\omega$ & $\omega$ & $\omega^2$ \\
$V_0$ & $2$ & $-2$ & $0$ & $1$ & $1$ & $-1$ & $-1$ \\
$V_1$ & $2$ & $-2$ & $0$ & $\omega$ & $\omega^2$ & $-\omega^2$ & $-\omega$ \\
$V_2$ & $2$ & $-2$ & $0$ & $\omega^2$ & $\omega$ & $-\omega$ & $-\omega^2$ \\
$W$   & $3$ & $3$ & $-1$ & $0$ & $0$ & $0$ & $0$ 
\end{tabular}
\end{center}


Observe that $V_0$ is the representation induced by $2T\subset \SL(2,\C)$. Then, the coefficients in \eqref{eq_formula_for_Ti} are computed as follows:

\begin{align*}
T_{\rho_0}&=\frac{1}{24\cdot (2-(-2))} + \frac{1}{4\cdot (2-0)} + \frac{1}{6\cdot (2-1)} +\\
& + \frac{1}{6\cdot (2-1) } + \frac{1}{6\cdot(2-(-1))} + \frac{1}{6\cdot (2-(-1))}=\frac{167}{288};\\
T_{\rho_1}=T_{\rho_2}&=\frac{1}{96}+ \frac{1}{8} +\frac{\omega}{6}+\frac{\omega^2}{6}+\frac{\omega}{18}+\frac{\omega^2}{18}=-\frac{25}{288};\\
T_{V_0}&= -\frac{2}{96}+ \frac{1}{6}+\frac{1}{6}-\frac{1}{18}-\frac{1}{18} = \frac{58}{288};\\
T_{V_1}=T_{V_2}&= -\frac{2}{96}+\frac{\omega}{6}+\frac{\omega^2}{6}- \frac{\omega}{18}-\frac{\omega^2}{18} = -\frac{38}{288};\\
T_{W}&=\frac{3}{96} - \frac{1}{8}=-\frac{27}{288}.
\end{align*}
We leave the analogous cases of singularities of type $E_7$ and $E_8$ to the reader.


\begin{comment}
The binary tetrahedral group has 7 conjugacy classes, with character table (https://ncatlab.org/nlab/show/tetrahedral+group). It has three characters, three rank 2 representations and one rank 3 one. Write
\[ [Li^*F]= \sum_{i=0}^2 a_i\chi^i + b_iV_i + cW. \]
The TRR terms are computed here
\begin{center}
\begin{tabular}{c|c|c|c}
Class $(g)$ & $\abs{C_G(g)}$ & $\widetilde{\mathrm{Td}_\sS}$ & $\widetilde{\ch{}}(F_g)$ \\
\hline
   $-I$ & 1 & 4 & $a_0+a_1+a_2 -2(b_0+b_1+b_2) + 3c$  \\
   $i$ & 4 & 2  & $a_0+a_1+a_2 -c$ \\
    $a$ & 6 & 3 & $a_0-b_0 +\omega(a_1+b_1)+ \omega^2(a_2+b_2)$  \\
    $b$ & 6 & 3  & $a_0 -b_0 +\omega^2(a_1+b_1) + \omega(a_2 + b_2)$ \\
    $c$&  6 & 1 & $a_0 + b_0 +\omega^2(a_1-b_1) +\omega(a_2-b_2)$  \\
    $d$ & 6 & 1 &  $a_0 + b_0 +\omega(a_1-b_1) +\omega^2(a_2-b_2)$ 
\end{tabular}
\end{center}
Then $\delta(\sF)$ is obtained by assembling the data in the table above...\AAA{maybe write down the $T_i$ for $E_6$, and call it a day.}
\end{comment}
